Learning 3D Robotics Perception using Inductive Priors

Recent advances in deep learning have led to a data-centric intelligence i.e. artificially intelligent models unlocking the potential to ingest a large amount of data and be really good at performing digital tasks such as text-to-image generation, machine-human conversation, and image recognition. This thesis covers the topic of learning with structured inductive bias and priors to design approaches and algorithms unlocking the potential of principle-centric intelligence. Prior knowledge (priors for short), often available in terms of past experience as well as assumptions of how the world works, helps the autonomous agent generalize better and adapt their behavior based on past experience. In this thesis, I demonstrate the use of prior knowledge in three different robotics perception problems. 1. object-centric 3D reconstruction, 2. vision and language for decision-making, and 3. 3D scene understanding. To solve these challenging problems, I propose various sources of prior knowledge including 1. geometry and appearance priors from synthetic data, 2. modularity and semantic map priors and 3. semantic, structural, and contextual priors. I study these priors for solving robotics 3D perception tasks and propose ways to efficiently encode them in deep learning models. Some priors are used to warm-start the network for transfer learning, others are used as hard constraints to restrict the action space of robotics agents. While classical techniques are brittle and fail to generalize to unseen scenarios and data-centric approaches require a large amount of labeled data, this thesis aims to build intelligent agents which require very-less real-world data or data acquired only from simulation to generalize to highly dynamic and cluttered environments in novel simulations (i.e. sim2sim) or real-world unseen environments (i.e. sim2real) for a holistic scene understanding of the 3D world.

==> chapters/nerfmae/05_qualitative.tex <==
\section{Qualitative Results}
\label{chap:nerfmae,sec:qualitative}

We qualitatively analyze the performance of NeRF-MAE on reconstruction, 3D OBB prediction, and voxel-labeling tasks. As shown in Figures~\ref{fig:qualitative_recon} and~\ref{fig:qualitative_recon_2}, our approach outputs plausible reconstructions faithful to the original input grid. This result shows our network's ability to find semantic and spatial relationships in the input data and understand the data distribution, which is useful for learning good representations for downstream tasks. We further show our networks' superior 3D OBB prediction performance in Figure~\ref{fig:qualitative_recon_3}. Our approach is able to reconstruct accurate bounding boxes where the state-of-the-art baseline struggles with incomplete or erroneous detections. Finally, we show our networks' superior semantic segmentation performance in Figure~\ref{fig:qualitative_recon_5}. This result further emphasizes our network learns good representations for posed 2D data and is able to excel in the challenging 3D segmentation task. 


==> tables/neo360/depth_metrics.tex <==
\setlength{\columnsep}{6pt}%
\begin{wraptable}{r}{0pt}
\scriptsize
\centering
\caption{Eval views depth prediction from 3 source views on NeRDS360}
\label{tab:depth_metrics}
\begin{tabular}{@{}lcc@{}}
\toprule
Object Depth & \textbf{L1} ↓ & \textbf{RMSE} ↓  \\ 
\midrule
PixelNeRF~\cite{yu2021pixelnerf} & 0.83 & 1.07  \\
NeRO~(no ft.) & 0.59 & 0.74\\
\midrule
~\textbf{NeRO~(Ours)}   & \textbf{0.20} & \textbf{0.61}\\
\bottomrule
\end{tabular}
\end{wraptable}

==> tables/shapo/ablation.tex <==
\setlength{\tabcolsep}{16pt}
\begin{table*}[t]
\centering
\large
\renewcommand{\arraystretch}{1.3}
\caption{\textbf{Ablation Study of Different LoDs on Downstream task of 3D object detection and 6D pose estimation}: Study of the Proposed CenterSnap method on NOCS Real-test set to investigate the impact of different components i.e. Input, Shape, Training Regime~(TR) and Depth-Auxiliary loss~(D-Aux) on performance. C indicates Camera-train, R indicates Real-train and RF indicates Real-train with finetuning. 3D shape reconstruction evaluated with \textbf{CD} ($10^{-2}$). $*$ denotes the method does not evaluate size and scale and so has no IOU metric.}
\label{tab:ablation}
\resizebox{1.0\textwidth}{!}{%
\begin{tabular}{c@{\hskip 0.1in}lccccccccc} \\
\toprule
& & & & \multicolumn{6}{c}{\textbf{Metrics}} \\ 
\cmidrule(r{0.05in}){6-6}
\cmidrule(r{0.05in}){7-10}

& & & & & \textbf{3D Shape} & \multicolumn{4}{c}{\textbf{6D Pose}} \\ 
% \cmidrule(){5-9}
\cmidrule(r{0.05in}){6-6}
\cmidrule(r{0.05in}){7-10}
 {\textbf{\#}} & \text{Shape Representation} &\text{LoD} &\text{Sparse(ICP)} & Dense(DR)&\textbf{CD}~$\downarrow$ & \textbf{IOU25}~$\uparrow$ & \textbf{IOU50}~$\uparrow$ &\textbf{5\textdegree \SI{10}{\cm}}~$\uparrow$ & \textbf{10\textdegree \SI{10}{\cm}}~$\uparrow$  \\

\midrule
 1 &PointCloud& - & C & \checkmark & 0.19 & 28.4 & 27.0 & 14.2 &48.2 \\
 2 &PointCloud& - & C+R & \checkmark & 0.19 & 41.5 & 40.1 & 27.1 & 58.2\\
 3 &Implicit& &LoD2 & \checkmark & --- & --- & --- & 13.8 & 50.2 \\
 4 & Implicit & LoD3 & \checkmark & \checkmark & 0.20 & 63.7 & 31.5 & 8.30 & 30.1\\
 5 &Implicit& LoD4 & C+RF & \checkmark & 0.15 & 74.2 & 66.7 & 30.2 & 63.2  \\
 6 &Implicit&LoD5  & C+RF&  & 0.17 & 82.3 & 78.3 & 30.8 &68.3 \\
 7 &Implicit& LoD6 & C+RF & \checkmark & 0.15 & 83.5 & 80.2 & 31.6 &70.9 \\
\bottomrule
\end{tabular}}

\end{table*}



==> vita.tex <==
% % Vita should only be included for PhD candidates.

% \begin{vita}

% Clark Kent was born on April 18, 1938, and adopted by parents Jonathan and Martha Kent in Kansas. He currently resides in the city of Metropolis, where his reporting for the Daily Planet has earned him critical acclaim both at home and abroad. He frequently collaborates with such fellow journalists as his Pulitzer-winning wife Lois Lane, close friend James ``Jimmy'' Olsen,  and longtime editor Perry White.

% Clark and Lois enjoy their quiet time together, when they can play with their dog and their teenage son, Jonathan.

% \end{vita}
